Source-Level Bitwise Branching for Temporal Verification

There is increasing interest in applying verification tools to programs that have bitvector operations. SMT solvers, which serve as a foundation for these tools, have thus increased support for bitvector reasoning through bit-blasting and linear arithmetic approximations. Still, verification tools are limited on termination and LTL verification of bitvector programs. In this work, we show that similar linear arithmetic approximation of bitvector operations can be done at the source level through transformations. Specifically, we introduce new paths that over-approximate bitvector operations with linear conditions/constraints, increasing branching but allowing us to better exploit the well-developed integer reasoning and interpolation of verification tools. We present two sets of rules, namely rewriting rules and weakening rules, that can be implemented as bitwise branching of program transformation, the branching path can facilitate verification tools widen verification tasks over bitvector programs. Our experiment shows this exploitation of integer reasoning and interpolation enables competitive termination verification of bitvector programs and leads to the first effective technique for LTL verification of bitvector programs.

==> abstractUpdate.tex <==
There is increasing interest in applying verification tools to programs that have bitvector operations. SMT solvers, which serve as a foundation for these tools, have thus increased support for bitvector reasoning through bit-blasting and linear arithmetic approximations. Still, verification tools are limited on termination and LTL verification of bitvector programs. %% \red{What is the problem here?}

In this \added{work}, we show that similar linear arithmetic approximation of bitvector operations can be done at the source level through transformations. Specifically, we introduce new paths that over-approximate bitvector operations with linear conditions/constraints, increasing branching but allowing us to better exploit the well-developed integer reasoning and interpolation of verification tools. We present two sets of rules, namely rewriting rules and weakening rules, that can be implemented as bitwise branching of program transformation, the branching path can facilitate verification tools widen verification tasks over bitvector programs. Our experiment shows this exploitation of integer reasoning and interpolation enables competitive termination verification of bitvector programs and leads to the first effective technique for LTL verification of bitvector programs.

Finally, for the cases that are not covered by our bitwise branching rules, we explore a dynamic approach combined with static analysis to tackle more complicated bitvector programs. We execute the program and collect concrete traces in the locations of interest, inferring program invariants from concrete traces, these linear invariants can be used to approximate the bitwise expressions, therefore the static analysis tools can reason about the approximate programs and return the verification results.  

